Joint Supervised and Self-supervised Learning for MRI Reconstruction

Magnetic Resonance Imaging (MRI) represents an important diagnostic modality; however, its inherently slow acquisition process poses challenges in obtaining fully-sampled $k$-space data under motion. In the absence of fully-sampled acquisitions, serving as ground truths, training deep learning algorithms in a supervised manner to predict the underlying ground truth image becomes challenging. To address this limitation, self-supervised methods have emerged as a viable alternative, leveraging available subsampled $k$-space data to train deep neural networks for MRI reconstruction. Nevertheless, these approaches often fall short when compared to supervised methods. We propose Joint Supervised and Self-supervised Learning (JSSL), a novel training approach for deep learning-based MRI reconstruction algorithms aimed at enhancing reconstruction quality in cases where target datasets containing fully-sampled $k$-space measurements are unavailable. JSSL operates by simultaneously training a model in a self-supervised learning setting, using subsampled data from the target dataset(s), and in a supervised learning manner, utilizing datasets with fully-sampled $k$-space data, referred to as proxy datasets. We demonstrate JSSL's efficacy using subsampled prostate or cardiac MRI data as the target datasets, with fully-sampled brain and knee, or brain, knee and prostate $k$-space acquisitions, respectively, as proxy datasets. Our results showcase substantial improvements over conventional self-supervised methods, validated using common image quality metrics. Furthermore, we provide theoretical motivations for JSSL and establish "rule-of-thumb" guidelines for training MRI reconstruction models. JSSL effectively enhances MRI reconstruction quality in scenarios where fully-sampled $k$-space data is not available, leveraging the strengths of supervised learning by incorporating proxy datasets.

==> tab_unet.tex <==
\begin{table}[!htb]
\centering
\caption{Average comparative metrics using an image domain U-Net architecture as a reconstruction network.}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{clccclccclccc}
\hline
\multirow{2}{*}{\textbf{Setup}} &  & \multicolumn{3}{c}{\textbf{4x}}                 &           & \multicolumn{3}{c}{\textbf{8x}}                 &           & \multicolumn{3}{c}{\textbf{16x}}                \\ \cline{3-5} \cline{7-9} \cline{11-13} 
                                &  & SSIM           & pSNR          & NMSE           &           & SSIM           & pSNR          & NMSE           &           & SSIM           & pSNR          & NMSE           \\ \cline{1-1} \cline{3-5} \cline{7-9} \cline{11-13} 
SSL                             &  & 0.854          & 33.0          & 0.013          &           & 0.742          & 29.4          & 0.030          &           & 0.651          & \textbf{26.7} & \textbf{0.055} \\
JSSL                            &  & \textbf{0.863} & \textbf{33.5} & \textbf{0.012} & \textbf{} & \textbf{0.759} & \textbf{29.7} & \textbf{0.027} & \textbf{} & \textbf{0.663} & 26.7          & 0.055          \\ \hline
\end{tabular}%
}
\label{tab:metrics_unet}
\end{table}

==> tab_varnet.tex <==
\begin{table}[!ht]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{clccclccclccc}
\hline
\multirow{2}{*}{\textbf{Setup}} &  & \multicolumn{3}{c}{\textbf{4x}}                 &           & \multicolumn{3}{c}{\textbf{8x}}                 &           & \multicolumn{3}{c}{\textbf{16x}}                \\ \cline{3-5} \cline{7-9} \cline{11-13} 
                                &  & SSIM           & pSNR          & NMSE           &           & SSIM           & pSNR          & NMSE           &           & SSIM           & pSNR          & NMSE           \\ \cline{1-1} \cline{3-5} \cline{7-9} \cline{11-13} 
SSL                             &  & 0.874          & 33.7          & 0.011          &           & 0.770          & 30.0          & 0.025          &           & 0.670          & 27.0          & 0.051          \\
JSSL                            &  & \textbf{0.888} & \textbf{34.9} & \textbf{0.008} & \textbf{} & \textbf{0.784} & \textbf{30.5} & \textbf{0.023} & \textbf{} & \textbf{0.678} & \textbf{27.1} & \textbf{0.050} \\ \hline
\end{tabular}%
}
\caption{Average comparative metrics using an E2EVarNet architecture as a reconstruction network.}
\label{tab:metrics_vnet}
\end{table}
